A Survey on Detection of LLMs-Generated Content

The burgeoning capabilities of advanced large language models (LLMs) such as ChatGPT have led to an increase in synthetic content generation with implications across a variety of sectors, including media, cybersecurity, public discourse, and education. As such, the ability to detect LLMs-generated content has become of paramount importance. We aim to provide a detailed overview of existing detection strategies and benchmarks, scrutinizing their differences and identifying key challenges and prospects in the field, advocating for more adaptable and robust models to enhance detection accuracy. We also posit the necessity for a multi-faceted approach to defend against various attacks to counter the rapidly advancing capabilities of LLMs. To the best of our knowledge, this work is the first comprehensive survey on the detection in the era of LLMs. We hope it will provide a broad understanding of the current landscape of LLMs-generated content detection, offering a guiding reference for researchers and practitioners striving to uphold the integrity of digital information in an era increasingly dominated by synthetic content. The relevant papers are summarized and will be consistently updated at https://github.com/Xianjun-Yang/Awesome_papers_on_LLMs_detection.git.

==> tables/main.tex <==
\begin{table*}[htbp]
\centering
\resizebox{0.96\textwidth}{!}
{
\begin{tabular}{cccc}
\hline
\textbf{\small{Categories}} & \textbf{\small{Source}} & \textbf{\small{Methods}} & \textbf{\small{Tested on}}  \\
\hline
\multirow{13}{*}{ Training-based }
 & \small{B} & GPTZero \citet{GPTZero} & ChatGPT, GPT-3, GPT-2, LLaMA, etc.  \\
 & \small{B} & OpenAI text classifier \citet{AITextClassifier} & 34 models from 5 different organizations  \\
 & \small{B} &  G$^3$Detector \citet{zhan2023g3detector} & GPT2-small, GPT2-large, GPT3.5-turbo, GPT4; BART-large, T5-large, GoogleTrans \\
 & \small{B} & \citet{bakhtin2019real} & TransfSmall, TransfBig, TransfHuge, GPT2 \\
 & \small{B} & \citet{ippolito-etal-2020-automatic} & GPT2-large \\
 & \small{B} & \citet{uchendu-etal-2020-authorship} & CTRL, GPT, GPT2, GROVER, XLM, XLNET, PPLM, FAIR \\
 & \small{B} & Ghostbuster \citet{verma2023ghostbuster} & gpt-3.5-turbo, text-davinci-003  \\
 &  \small{B} & GPT-Pat \citet{yu2023gpt} & ChatGPT  \\
 & \small{B} & GPT-Sentinel \citet{chen2023gpt} & ChatGPT  \\
 %& \small{B} & \citet{becker2023paraphrase} & machine-paraphrase or back-translation using small LLM like BERT  \\
 & \small{B} & \citet{krishna2023paraphrasing} & GPT2-1.5B, OPT-13B, GPT-3.5-175B-davinci-003  \\
 & \small{B} & LLMDet \citet{wu2023llmdet} &  GPT2, GPT-2-Large, OPT-1.3B, OPT-2.7B, UniLM, LLaMA-7B, BART, T5-Base, Bloom-650M, GPTNeo-2.7B, Vicuna-7B  \\
& \small{B} & \citet{tian2023multiscale} & ChatGPT  \\
& \small{B} & \citet{deng2023efficient} & LLaMA-65B, GPT-2  \\

 
\hline

\multirow{6}{*}{ Watermarking} 
 & \small{W} & \citet{kirchenbauer2023watermark} & OPT-1.3, 2.7, 6.7 \\
 & \small{B} & \citet{yang2023watermarking} & ChatGPT-3.5  \\
 & \small{W} &  Undetectable Watermarks \citet{christ2023undetectable} & Only theoretical analysis  \\
 & \small{W} & AWT\citet{abdelnabi21oakland} & SBERT \\
 & \small{W} & \citet{yoo2023robust} & Theoretical analysis on BERT-base \\
 & \small{W} & \citet{tang2023baselines} & Flan-T5-XXL, Alpaca-LoRA \\
& \small{B} & \citet{yang2022tracing} & bert-base-cased, roberta-large-mnli \\
& \small{B} & \citet{kirchenbauer2023reliability} & Llama, Vicuna, gpt-3.5-turbo, 11B Dipper \\
\hline

\multirow{5}{*}{ Zero-shot }
 & \small{W} & DetectGPT \citet{mitchell2023detectgpt} &  GPT-2, OPT-2.7, Neo-2.7, GPT-J, NeoX, GPT-3  \\
 & \small{B, W} & DNA-GPT \citet{yang2023dna} & GPT-3, 3.5, 4, LLaMa-13, NeuoX-20 \\
 & \small{B, W} & Cross-detection \citet{mireshghallah2023smaller} & OPT, EleutherAI, OpenAI’s GPT families  \\

 & \small{B} &  PHD \citet{tulchinskii2023intrinsic} & GPT3.5-turbo, GPT2-XL, OPT-13b, GPT3.5-davinci-003 \\

& \small{W} &  DetectLLM \citet{su2023detectllm} & GPT2-xl, Neo-2.7, OPT-2.7, GPT-J, OPT-13, LLama-13, NeoX \\



\hline
\end{tabular}
}
\caption{An overview of three categories of detectors. W, B represent White-box and Black-box about the source model, respectively. \xd{It makes more sense to summerize the method instead of listing the tested models as the last column.}}\label{table:main}
\end{table*}\vspace{-0.3cm}

% & \small{W} & \small{ DetectLLM \citet{su2023detectllm}} & \small{GPT2-xl, Neo-2.7, OPT-2.7, GPT-J, OPT-13, Llama-13, NeoX} & \small{-} \\

%  & \small{B} & \small{ \citet{}} & \small{-} & \small{-} \\

==> tables/main2.tex <==

\begin{table*}[htbp]
\centering
\label{tab:methods}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Categories} & \textbf{Models} & \textbf{Methods} & \textbf{Tested on} \\
\hline
\multirow{2}{*}{Training-based} & White-box & \parbox{4cm}{Details of M1, White-box Details of M1, White-box Details of M1, White-box} & sd \\
\cline{2-4}
 & Black-box & \parbox{4cm}{Details of M1, Black-box} & sd\\
\hline
\multirow{2}{*}{Watermarking} & White-box & \parbox{4cm}{Details of M2, White-box Details of M2, White-box Details of M2, White-box} & ss \\
\cline{2-4}
 & Black-box & \parbox{4cm}{Binary Encoding \citet{yang2023watermarking}} & ss\\
\hline
\multirow{2}{*}{Zero-shot} & White-box & \parbox{4cm}{DetectGPT \citet{mitchell2023detectgpt}, DNA-GPT \citet{yang2023dna} } &  \parbox{4cm}{Details of M3, White-box} \\
\cline{2-4}
 & Black-box & \parbox{4cm}{Cross detection \citet{mireshghallah2023smaller}, } & \parbox{4cm}{Details of M3, White-box} \\
\hline
\end{tabular}\label{table:main}
\caption{An overview of three categories of detectors. }
\end{table*}


% \begin{table*}[htbp]
% \centering
% \label{tab:methods}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Categories} & \textbf{Models} & \textbf{Methods} & \textbf{Tested on} \\
% \hline
% \multirow{2}{*}{Training-based} & White-box & Details of M1, White-box Details of M1, White-box Details of M1, White-box& \multirow{2}{*}{Models for M1} \\
% \cline{2-3}
%  & Black-box & Details of M1, Black-box & \\
% \hline
% \multirow{2}{*}{Watermarking} & White-box & Details of M2, White-box & \multirow{2}{*}{Models for M2} \\
% \cline{2-3}
%  & Black-box & Details of M2, Black-box & \\
% \hline
% \multirow{2}{*}{Zero-shot} & White-box & Details of M3, White-box &  Details of M3, White-box \\
% %\multirow{2}{*}{Models for M3} \\
% \cline{2-3}
%  & Black-box & Details of M3, Black-box & Details of M3, White-box \\
% \hline
% \end{tabular}\label{table:main}
% \caption{An overview of three categories of detectors. }
% \end{table*}



==> tables/temp.tex <==
\begin{table*}[htbp]
\centering
\resizebox{0.96\textwidth}{!}
{
\begin{tabular}{ccccc}
\hline
\textbf{\small{Categories}} & \textbf{\small{Source}} & \textbf{\small{Methods}} & \textbf{\small{Tested on}} & \textbf{\small{Cost}} \\
\hline
\multirow{14}{*}{ Training-based }
 & \small{B} & GPTZero \citet{GPTZero} & ChatGPT, GPT-3, GPT-2, LLaMA, etc. & \small{-} \\
 & \small{B} & OpenAI text classifier \citet{AITextClassifier} & 34 models from 5 different organizations & \small{-} \\
 & \small{B} &  G$^3$Detector \citet{zhan2023g3detector} & GPT2-small, GPT2-large, GPT3.5-turbo, GPT4; BART-large, T5-large, GoogleTrans & \small{-} \\
 & \small{B} & \citet{bakhtin2019real} & TransfSmall, TransfBig, TransfHuge, GPT2& \small{-}\\
 & \small{B} & \citet{ippolito-etal-2020-automatic} & GPT2-large& \small{-}\\
 & \small{B} & \citet{uchendu-etal-2020-authorship} & CTRL, GPT, GPT2, GROVER, XLM, XLNET, PPLM, FAIR & \small{-}\\
 & \small{B} & Ghostbuster \citet{verma2023ghostbuster} & gpt-3.5-turbo, text-davinci-003 & \small{-}\\
 &  \small{B} & GPT-Pat \citet{yu2023gpt} & ChatGPT & \small{2}\\
 & \small{B} & GPT-Sentinel \citet{chen2023gpt} & ChatGPT & \small{-}\\
 & \small{B} & \citet{becker2023paraphrase} & machine-paraphrase or back-translation using small LLM like BERT & \small{-}\\
 & \small{B} & \citet{krishna2023paraphrasing} & GPT2-1.5B, OPT-13B, GPT-3.5-175B-davinci-003 & \small{-}\\
 & \small{B} & LLMDet \citet{wu2023llmdet} &  GPT2, GPT-2-Large, OPT-1.3B, OPT-2.7B, UniLM, LLaMA-7B, BART, T5-Base, Bloom-650M, GPTNeo-2.7B, Vicuna-7B & \small{-}\\
& \small{B} & \citet{tian2023multiscale} & ChatGPT & \small{-}\\
& \small{B} & \citet{deng2023efficient} & LLaMA-65B, GPT-2 & \small{-}\\

 
\hline

\multirow{6}{*}{ Watermarking} 
 & \small{W} & \citet{kirchenbauer2023watermark} & OPT-1.3, 2.7, 6.7 & \small{1} \\
 & \small{B} & \citet{yang2023watermarking} & ChatGPT-3.5 & \small{-} \\
 & \small{W} &  Undetectable Watermarks \citet{christ2023undetectable} & Only theoretical analysis & \small{-} \\
 & \small{W} & AWT\citet{abdelnabi21oakland} & SBERT & \small{-}\\
 & \small{W} & \citet{yoo2023robust} & BERT-base & \small{-}\\
 & \small{W} & \citet{tang2023baselines} & Flan-T5-XXL, Alpaca-LoRA & \small{-}\\
& \small{B} & \citet{yang2022tracing} & bert-base-cased, roberta-large-mnli& \small{-}\\
& \small{B} & \citet{kirchenbauer2023reliability} & Llama, Vicuna, gpt-3.5-turbo, 11B Dipper  & \small{1}\\
\hline

\multirow{5}{*}{ Zero-shot }
 & \small{W} & DetectGPT \citet{mitchell2023detectgpt} &  GPT-2, OPT-2.7, Neo-2.7, GPT-J, NeoX, GPT-3 & \small{100N} \\
 & \small{B, W} & DNA-GPT \citet{yang2023dna} & GPT-3, 3.5, 4, LLaMa-13, NeuoX-20 & \small{10N} \\
 & \small{B, W} & Cross-detection \citet{mireshghallah2023smaller} & OPT, EleutherAI, OpenAI’s GPT families & \small{100N} \\

 & \small{B} &  PHD \citet{tulchinskii2023intrinsic} & GPT3.5-turbo, GPT2-XL, OPT-13b, GPT3.5-davinci-003,  & \small{-} \\

& \small{B} &  DetectLLM \citet{su2023detectllm} & GPT2-xl, Neo-2.7, OPT-2.7, GPT-J, OPT-13, LLama-13, NeoX & \small{-} \\



\hline
\end{tabular}
}
\caption{An overview of three categories of detectors. W, B represent White-box and Black-box about the source model, respectively.}\label{table:main}
\end{table*}\vspace{-0.3cm}

% & \small{W} & \small{ DetectLLM \citet{su2023detectllm}} & \small{GPT2-xl, Neo-2.7, OPT-2.7, GPT-J, OPT-13, Llama-13, NeoX} & \small{-} \\

%  & \small{B} & \small{ \citet{}} & \small{-} & \small{-} \\
